MOrdReD: Memory-based Ordinal Regression Deep Neural Networks for Time Series Forecasting

Time series forecasting is ubiquitous in the modern world. Applications range from health care to astronomy, and include climate modelling, financial trading and monitoring of critical engineering equipment. To offer value over this range of activities, models must not only provide accurate forecasts, but also quantify and adjust their uncertainty over time. In this work, we directly tackle this task with a novel, fully end-to-end deep learning method for time series forecasting. By recasting time series forecasting as an ordinal regression task, we develop a principled methodology to assess long-term predictive uncertainty and describe rich multimodal, non-Gaussian behaviour, which arises regularly in applied settings. Notably, our framework is a wholly general-purpose approach that requires little to no user intervention to be used. We showcase this key feature in a large-scale benchmark test with 45 datasets drawn from both, a wide range of real-world application domains, as well as a comprehensive list of synthetic maps. This wide comparison encompasses state-of-the-art methods in both the Machine Learning and Statistics modelling literature, such as the Gaussian Process. We find that our approach does not only provide excellent predictive forecasts, shadowing true future values, but also allows us to infer valuable information, such as the predictive distribution of the occurrence of critical events of interest, accurately and reliably even over long time horizons.

==> vitae.tex <==
\begin{footnotesize}

\textbf{Bernardo P\'erez Orozco} is a current DPhil (PhD) student at the University of Oxford's Machine Learning Research Group under Prof. Steve Roberts. His research is focused on enabling deep recurrent neural network architectures to perform time series forecasting in a probabilistic and interpretable fashion. Bernardo is passionate about the connection between Statistics and Computer Science in both applied and theoretical settings. He holds a Master of Science in Computer Science from the University of Oxford and previously read for a degree in Computer Systems Engineering at Tecnol\'ogico de Monterrey, Campus Quer\'etaro in Mexico.


\textbf{Gabriele Abbati} a second year D.Phil. (Ph.D.) candidate in the Machine Learning Research Group at the University of Oxford, supervised by Michael Osborne. His research interests within Machine Learning and Artificial Intelligence are broad and include topics such as Bayesian frameworks for Deep Learning, Bayesian Neural Networks and Gaussian Processes. Gabriele holds a Master of Science in Computational Science and Engineering from ETH Zurich and a Bachelor of Engineering in Mathematical Engineering from Politecnico di Milano.


\textbf{Stephen Roberts} is the Royal Academy of Engineering/Man Group Professor of Machine Learning at the University of Oxford. He is a Fellow of the Royal Academy of Engineering, the Royal Statistical Society, the Institute of Physics and is a Faculty Fellow of the Alan Turing Institute. Stephen is Director of the Oxford-Man Institute of Quantitative Finance. His current major interests include the application of machine learning to astrophysical data sets, biodiversity monitoring, smart networks, sensor networks and finance. 

\end{footnotesize}
